Discovery of a Jupiter Analog Misaligned to the Inner Planetary System in HD 73344

We present the discovery of a Jupiter-like planet, HD 73344 d ($m_{d}=2.55^{+0.56}_{-0.46}\ \mathrm{M_{J}}$, $a_{d}=6.70^{+0.25}_{-0.26}$ AU, $e_{d}=0.18^{+0.14}_{-0.12}$) based on 27-year radial velocity observations. HD 73344 also hosts a compact inner planetary system, including a transiting sub-Neptune HD 73344 b ($P_{b}=15.61\ \mathrm{days}$, $r_{b}=2.88^{+0.08}_{-0.07}\ \mathrm{R_{\oplus}}$) and a non-transiting Saturn-mass planet ($P_{c}=65.936\ \mathrm{days}$, $m_{c}\sin{i_c}=0.36^{+0.02}_{-0.02}\ \mathrm{M_{J}}$). By analyzing TESS light curves, we identified a stellar rotation period of $9.03\pm{1.3}$ days. Combining this with $v\sin{i_*}$ measurements from stellar spectra, we derived a stellar inclination of $63.6^{+17.4}_{-16.5}\ \rm{deg} $. Furthermore, by combining radial velocities and Hipparcos-Gaia astrometric acceleration, we characterized the three-dimensional orbit of the outer giant planet and constrained its mutual inclination relative to the innermost transiting planet to be $46 <\Delta I_{bd}< 134\ \rm{deg}\ (1\sigma)$ and $20 <\Delta I_{bd}< 160\ \rm{deg}\ (2\sigma)$, strongly disfavoring coplanar architectures. Our analytical calculations and N-body simulation reveal that the two inner planets are strongly coupled with each other and undergo nodal precession together around the orbital axis of the giant planet. During nodal precession, the orbital inclination of inner planets oscillate with time and therefore become misaligned relative to the stellar spin axis. The formation of such systems suggests a history of planet-planet scattering or misalignment between the inner and outer components of protoplanetary disks. The upcoming release of Gaia DR4 will uncover more systems similar to HD 73344 and enable the study of the flatness of exoplanet systems with a mixture of inner and outer planetary systems on a statistical level.

==> tabe_radvel_keep.tex <==
\begin{deluxetable}{lrrrr}
\tablecaption{ MCMC Posteriors for RV-only fitting}\label{tab:rvparams}
\tablehead{
  \colhead{Parameter} & 
  \colhead{ Median$\pm{1\sig}$} & 
  \colhead{Best-fit} & 
  \colhead{Units} & 
  \colhead{Prior}
}
\startdata
\multicolumn{4}{c}{\bf{Fitted parameters}} \\[1pt]
\hline
  $P_{b}$ & $15.604^{+0.044}_{-0.036}$ & $15.6$ & days & $\mathcal{N}(15.60 ,0.05)$  \\
  $T\rm{conj}_{b}$ & $2458484.6^{+1.1}_{-1.0}$ & $2458484.7$ & JD \\
  $e_{b}$ & $\equiv0.0$ & $\equiv0.0$ &  \\
  $\omega_{b}^{\dagger}$ & $\equiv0.0$ & $\equiv0.0$ & radians \\
  $K_{b}$ & $<2.82\ (3\sigma)$ & $0.44$ & m s$^{-1}$ \\
  $P_{c}$ & $65.936^{+0.023}_{-0.022}$ & $65.936$ & days \\
  $T\rm{conj}_{c}$ & $2455482.98^{+0.92}_{-0.89}$ & $2455483.01$ & JD \\
  $e_{c}$ & $0.124^{+0.052}_{-0.053}$ & $0.128$ &  \\
  $\omega_{c}^{\dagger}$ & $1.96^{+0.43}_{-0.41}$ & $-1.18$ & radians \\
  $K_{c}$ & $16.83\pm 0.87$ & $16.8$ & m s$^{-1}$ \\
  $P_{d}$ & $5746^{+170}_{-150}$ & $5699$ & days \\
  $T\rm{conj}_{d}$ & $2444345^{+100}_{-550}$ & $2444325$ & JD \\
  $e_{d}$ & $0.2\pm{0.1}$ & $0.175$ &  \\
  $\omega_{d}^{\dagger}$ & $1.07^{+0.62}_{-0.58}$ & $-1.99$ & radians \\
  $K_{d}$ & $22.7\pm 3.4$ & $23.4$ & m s$^{-1}$ \\
\hline
\multicolumn{4}{c}{\bf{Other parameters}} \\[1pt]
\hline
  $\gamma_{\rm ELODIE}$ & $\equiv6223.9168$ & $\equiv6223.9168$ & m s$-1$ \\
  $\gamma_{\rm Lick\ Fischer}$ & $\equiv-14.7772$ & $\equiv-14.7772$ & m s$-1$ \\
  $\gamma_{\rm HIRES}$ & $\equiv-2.0331$ & $\equiv-2.0331$ & m s$-1$ \\
  $\gamma_{\rm APF}$ & $\equiv0.0938$ & $\equiv0.0938$ & m s$-1$ \\
  $\gamma_{\rm SOPHIE}$ & $\equiv6235.7652$ & $\equiv6235.7652$ & m s$-1$ \\
  $\dot{\gamma}$ & $\equiv0.0$ & $\equiv0.0$ & m s$^{-1}$ d$^{-1}$ \\
  $\ddot{\gamma}$ & $\equiv0.0$ & $\equiv0.0$ & m s$^{-1}$ d$^{-2}$ \\
  $\sigma_{\rm ELODIE}$ & $16.7^{+2.6}_{-2.2}$ & $16.0$ & $\rm m\ s^{-1}$ \\
  $\sigma_{\rm Lick\ Fischer}$ & $25.3^{+5.3}_{-4.0}$ & $24.0$ & $\rm m\ s^{-1}$ \\
  $\sigma_{\rm HIRES}$ & $9.65^{+0.26}_{-0.48}$ & $10.0$ & $\rm m\ s^{-1}$ \\
  $\sigma_{\rm APF}$ & $19.8^{+3.8}_{-2.8}$ & $19.1$ & $\rm m\ s^{-1}$ \\
  $\sigma_{\rm SOPHIE}$ & $11.76^{+0.51}_{-0.5}$ & $11.63$ & $\rm m\ s^{-1}$ \\
\hline
\multicolumn{4}{c}{\bf{Derived parameters}} \\[1pt]
\hline
  $M_b$ & $<12.43\ (3\sigma)$ & $0.5$ & M$_{\oplus}$ \\
  $a_b$ & $0.1296^{+0.0016}_{-0.0017}$ & $0.1325$ &  AU \\
  $M_c\sin i$ & $0.373^{+0.022}_{-0.021}$ & $0.373$ & M$_{\rm Jup}$ \\
  $a_c$ & $0.3388^{+0.0042}_{-0.0043}$ & $0.3463$ &  AU \\
  $M_d\sin i$ & $2.21^{+0.34}_{-0.35}$ & $2.03$ & M$_{\rm Jup}$ \\
  $a_d$ & $6.66^{+0.16}_{-0.15}$ & $6.9$ &  AU \\
\hline
\enddata
\tablenotetext{}{$\dagger$ The default output from RadVel is the argument of periastron for the star. Here, we report the argument of periastron for the planets by adding an offset of $\pi$. }
\label{tab:params}
\end{deluxetable}

==> test.tex <==
\begin{deluxetable}{lcc}
\tabletypesize{\small}
\tablecaption{MCMC posteriors for three-dimensional orbit fitting of HD 73344 d\label{tab:ch3_3d}}
\setlength{\tabcolsep}{0.10in}
\tablewidth{0pt}
\tablehead{
\colhead{Parameter (Unit)}              &
\colhead{Median $\pm$1$\sigma$} &
\colhead{Prior}                 }
\startdata
\multicolumn{3}{c}{Fitted parameters} \\[1pt]
\hline
\multicolumn{3}{c}{} \\[-5pt]
RV semi-amplitude of 73344~c $K_{c}$ ($\mathrm{m\,s^{-1}}$)                                      & $16.36^{+1.15}_{-1.12}$                      & no prior                                                \\[3pt]
Orbital periods $P_{c}$ (days)                                                     & $65.94\pm{0.02}$                & $\mathcal{N}(66 , 1)$                                                   \\[3pt]
Eccentricity term$\sqrt{e_c}\cos{\omega_{c}}$                                                      & $0.06^{+0.18}_{-0.20}$            & no prior                                                            \\[3pt]
Eccentricity term$\sqrt{e_{c}}\sin{\omega_{c}}$                                                      & $-0.24^{+0.20}_{-0.12}$              & no prior                                                           \\[3pt]
Epoch of periastron at 2454574.5 JD,  $\tau_{\rm c}$ & $0.35^{+0.15}_{-0.14}$                         & no prior       \\[3pt]

Planet mass $m_{\rm d}$ ($\mathrm{M_{J}}$)                                       & $2.55^{+0.56}_{-0.46}$                           & no prior                                                 \\[3pt]
Orbital periods $P_{d}$ (days)                                                     & $5823_{-308}^{+312}$                &  no prior                                                    \\[3pt]
Cosine term of inclination $\cos{I_{d}}^{1}$                                                   & $-0.63_{-0.22}^{+0.18}$              &  no prior                              \\[3pt]
Longitude of ascending node  $\Omega_{d}$  (deg)                                &  $144_{+55}^{-43}$                &  no prior                                                             \\[3pt]
Eccentricity term$\sqrt{e}_{d}\cos{\omega_{d}}$                                                    & $-0.20^{+0.30}_{-0.27}$               &  no prior                              \\[3pt]
Eccentricity term$\sqrt{e_{d}}\sin{\omega_{d}}$                                          
            &  $-0.27^{+0.34}_{-0.20}$              &  no prior                                                            \\[3pt]
Epoch of periastron at 2454574.5 JD, $\tau_{\rm c}$ & $0.59^{+0.12}_{-0.17}$                       &  no prior         \\[3pt]
Host-star mass $M_{*}$ ($\mathrm{M_{\odot}}$)                                       & $1.18\pm0.05$                      & $\mathcal{N}(1.18 ,0.09)$                                                    \\[3pt]
Parallax $\varpi$ (mas)                                                              & $23.38\pm0.02$                          & $\mathcal{N}(\varpi_{\rm DR3} ,\sigma[\varpi_{\rm DR3}])^{2}$ \\[3pt]
RV zero point $\gamma_{\rm{SOPHIE}}$($\mathrm{m\,s^{-1}}$ )                                      &$6236.93^{+5.09}_{-4.91}$                     & no prior                                                            \\[3pt]
RV zero point $\gamma_{\rm{ELODIE}}$($\mathrm{m\,s^{-1}}$ )                                      &$6221.95^{+4.55}_{-4.73}$                     & no prior                                                            \\[3pt]
RV zero point $\gamma_{\rm{HIRES}}$($\mathrm{m\,s^{-1}}$ )                                      &       $-0.98^{+4.56}_{-3.95}$                       & no prior                                                            \\[3pt]
RV zero point $\gamma_{\rm{APF}}$($\mathrm{m\,s^{-1}}$ )                                      &$-0.20^{+5.88}_{-5.15}$                     & no prior                                                            \\[3pt]
RV zero point $\gamma_{\rm{lick\ fischer}}$($\mathrm{m\,s^{-1}}$ )                                      &       $-13.52^{+5.46}_{-5.32}$                       & no prior                                                            \\[3pt]
RV jitter term $\sigma_{\rm{SOPHIE}}$($\mathrm{m\,s^{-1}}$)                                      &     $11.81^{+0.76}_{-0.70}$                       & $\mathcal{U}(0,25)$                                                           \\[3pt]
RV jitter term $\sigma_{\rm{ELODIE}}$($\mathrm{m\,s^{-1}}$)                                      &     $16.49^{+2.32}_{-2.15}$                       & $\mathcal{U}(0,25)$                                                           \\[3pt]
RV jitter term $\sigma_{\rm{HIRES}}$($\mathrm{m\,s^{-1}}$)                                      & $11.96^{+1.62}_{-1.33}$                            & $\mathcal{U}(0,25)$                                                           \\[3pt]
RV jitter term $\sigma_{\rm{APF}}$($\mathrm{m\,s^{-1}}$)                                      &     $18.08^{+2.91}_{-2.37}$                       & $\mathcal{U}(0,25)$                                                           \\[3pt]
RV jitter term $\sigma_{\rm{lick\ fisher}}$($\mathrm{m\,s^{-1}}$)                                      & $23.69^{+3.48}_{-3.33}$                            & $\mathcal{U}(0,25)$                                                           \\[3pt]
\hline
\multicolumn{3}{c}{} \\[-5pt]
\multicolumn{3}{c}{Derived parameters }\\[1pt]
\hline
\multicolumn{3}{c}{} \\[-5pt]
$\rm{Inclination}$ $I_{d}^{1}$ (deg)                                   & $58_{-16}^{+19}$                & no prior                                                            \\[3pt]
Semi-major axis $a_{d}$ (AU)                                                     & $6.70_{-0.26}^{+0.25}$                             & no prior                                                            \\[3pt]
Eccentricity $e_{d}$                                                            & $0.18^{+0.14}_{-0.12}$                 & $\mathcal{U}(0,0.99)$                                                            \\[3pt]
Argument of periastron $\omega_{d}$ (deg$)^{3}$                                   & $58.9_{-79.0}^{+57.3}$                & no prior                                                            \\[3pt]
Time of periastron $T_{p,c}$ (JD) & $2458061_{-1148}^{+735}$    & no prior                                                            \\
\enddata
\tablecomments{ 1. There are double peaks in the distribution of inclination due to the pro-grade and retro-grade degeneracy. We only present the solutions with $I_{d}>90^{\circ}$ here. 2.$\varpi_{\rm DR3}$ and $\sigma[\varpi_{\rm DR3}]$ present the parallax and parallax uncertainty of HD 118203 from Gaia DR3 observations. 3. We report the periastron of argument for planets here.} %5. The HIRES RVs are median-subtracted, whereas the ELODIE RVs are not.1.The $\chi^{2}$ of RVs is 77 for 80 measurements. }
\end{deluxetable}
